Recovering Grammar Relationships for the Java Language Specification

Grammar convergence is a method that helps discovering relationships between different grammars of the same language or different language versions. The key element of the method is the operational, transformation-based representation of those relationships. Given input grammars for convergence, they are transformed until they are structurally equal. The transformations are composed from primitive operators; properties of these operators and the composed chains provide quantitative and qualitative insight into the relationships between the grammars at hand. We describe a refined method for grammar convergence, and we use it in a major study, where we recover the relationships between all the grammars that occur in the different versions of the Java Language Specification (JLS). The relationships are represented as grammar transformation chains that capture all accidental or intended differences between the JLS grammars. This method is mechanized and driven by nominal and structural differences between pairs of grammars that are subject to asymmetric, binary convergence steps. We present the underlying operator suite for grammar transformation in detail, and we illustrate the suite with many examples of transformations on the JLS grammars. We also describe the extraction effort, which was needed to make the JLS grammars amenable to automated processing. We include substantial metadata about the convergence process for the JLS so that the effort becomes reproducible and transparent.

==> cover.tex <==
\newpage

\section*{Dear editors, dear (SCAM'09) reviewers,}

\bigskip

in the following, we reply to the SCAM 2009 reviews. This reply may
serve as a good description of the revision, too. Upfront, we
mention the following efforts to add material.

\section*{Added material (compared to SCAM'09 initial\&final version}

\begin{itemize}

\item Added a description of the transformation suite.
\item Added a new section on the extraction part of the study.
\item Doubled the coverage of transformation operators and
  corresponding scenarios.
\item Added a comparison of the transformation operators with prior
  art.
\item Aggressively extended related-work discussion.
\end{itemize}

\bigskip

\section*{Per-review replies}

\begin{itemize}

\item Review 1

\begin{itemize}

  \qa{This is very nice work, clearly useful in an important area.  We
    all wish that the JLS authors had had access to such a tool! My
    main reservation is that the well-reported case study is presented
    without enough context about the earlier work (and overall
    direction of the research) to help the reader understand all the
    implications of the study.%
  }{%
    The introduction has been rewritten from scratch to address this
    context problem. There is also a new section generally on grammar
    convergence. This makes the paper more self-contained, too.}

  \qa{Specific comments%
  }{%
    Done.}

\end{itemize}

\medskip

\item Review 2

\begin{itemize}

  \qa{I am not an expert in grammar(ware) engineering. Indeed, I did
    not know this phrase before reading the paper for this
    review. However, I have to say that as a (hopefully informed)
    outsider, I found this to be an interesting and very valuable
    paper (even an exciting paper, and that is quite high praise given
    that I come as an outsider and in our field outsiders seldom get
    excited about work not in their own field!). I also thought that
    the underlying philosophy, as I understand it, of grammarware
    engineering is a very sensible and timely one. I believe that
    grammars are increasingly important and that understanding the
    relationships between them is also very valuable and important
    work that deserves to be regarded as an important form of
    meta-SCAM. I have not kept pace with all the recent developments
    in parsing techniques, though I have been previously inspired by
    (one of) the authors work on island grammars and so I would defer
    to other referees concerning the novelty of this work. However, I
    would say that I personally found it to be a most interesting use
    of grammar transformation technology and I certainly have not seen
    work like this before. The authors claim originality and give a
    very compelling and cogent account of related work and I have no
    reason at all to doubt them on this point. The paper will be very
    useful to those who use Java (clearly) and also to language
    designers.
  }{%
    Thank you!}

  \qa{It occurred to me that the approach could be combined with
    grammar extraction techniques that capture coding styles of
    different programmers to explore the relationship between
    programmers and sets or teams of programmers.  Since I have little
    of value to say about the paper other than I feel that it is very
    exciting and important and should be accepted, I will spend a
    little time explaining this idea in case it is of interest to the
    authors. This is merely my attempt to add value with what would,
    otherwise, be a rather short (though positive) review!  I wonder
    whether the authors have come across the work of Di Penta et
    al. on SBSE techniques for inferring sub- grammars from examples?
    This work essentially uses search based optimization to extract
    from a grammar and sets of instances, a subgrammar (actually
    specialized would be a better word, since the extracted grammar is
    not a "subset" of the production rules of the original). The
    extracted grammar captures the nuances of the programmers in a
    very clever way It allows us to understand and document the
    idiosyncrasies of the programmers and also to explore their
    implicit guidelines on coding styles and such like. One can even,
    potentially, see how different programmers implement (or fail to)
    coding standards using this approach. One of the pleasing aspects
    is that it is all automated, since it uses SBSE to extract the
    specialised grammar from the programmers' code.  If the authors
    are interested there are tow papers (and CMSR paper and a
    subsequent journal version) ... I was thinking that, based on this
    work, the authors approach could be applied as a complement to
    explore the relationships between the grammars found for different
    groups of programmers. We could extract various specialized
    grammars from sets of real coders (this has been done by Di Penta
    et al. I believe, or it could be using their approach) and then,
    we could us the authors' approach to understand the relationships
    between these coding styles. It may seem a bit of a leap, but this
    could have a number of interesting applications. Clearly it would
    be interesting in and of itself, to understand these
    relationships. However, we could also identify those programmers
    who have most opposing styles (perhaps in pair programming or
    other co-working situations these two programmers, or groups of
    programmers, should not be paired!). Also we could see how the
    same programmer evolved their style by extracting grammars (using
    the Di Penta approach) over time and using the Laemmel and Zaytsev
    approach to understand their evolution.  I hope that the authors
    find this idea interesting and that it make an otherwise rather
    dull but appreciative review a little more valuable to them.%
  }{%
    Yes, we did not know of this work, but it is indeed interesting to
    compare, and perhaps, in the future, to combine the SBSE approach
    and the convergence approach. The revised, related work discussion
    goes into this direction; see the paragraph on grammar inference,
    where we discuss Di Penta et al.'s approach as much as other work
    on grammar inference.}

\end{itemize}

\medskip

\item Review 3

\begin{itemize}

  \qa{The paper is nice, though it is not quite clear how it improves
    over their earlier work.%
  }{%
    The reviewer presumably refers to previous work on operator suites
    for grammar transformation, as we used them for grammar recovery
    in particular. The revision has a very much extended related work
    discussion that addresses both improvements of our current work
    over earlier on transformation operators and the method for
    grammar recovery. For instance, we analyses the different operator
    suites and included a table that shows the different coverage; see
    related work section. However, we would like to emphasize that the
    main contribution of the present paper is one that is based on a
    specific (and challenging) study: JLS, and a nontrivial refinement
    of grammar convergence. The process of grammar convergence is
    comparison-based as opposed to parsing-based in our previous work
    on grammar transformation and recovery.%
  }

  \qa{In general the presentation seems somewhat light-weight compared
    to what they could present.%
  }{%
    We have added more technical meat. In particular: conceptual and
    technical details for grammar extraction; a precise list of all
    grammar transformation operators; archetypal examples for most of
    them based on the JLS study; details of grammar comparison.%
  }

  \qa{%
    I would like to see a complete presentation of their algebra of
    grammar transformations, and proofs of the claimed properties of
    these (section 3).%
  }{%
    The reviewer presumably notices that this expectation is very
    substantial here. Formalizing XBGF with its rich operator suite
    based on a rich metasyntax is a complex task. XBGF is programmed
    rather declaratively in about 100KB of Prolog. A specification,
    yet without proofs, is likely to be of that size. A mechanized
    proof would require enormous resources. We are investigating this
    overall question on how better formalize XBGF, without causing man
    years of work, but this is ongoing thinking. Obviously we would
    need to identify a core XBGF language and start from there. But
    again, it would really go beyond the current paper, which is about
    a study and a method, to formalize XBGF.%
  }

  \qa{It would also be useful if the authors would elaborate more on
    their experience on how to evolve languages and grammars. They
    have some side comments hinting on useful guidelines, but it
    should be possible to elaborate this.%
  }{%
    We have added a short paragraph at the very end of Section 4. We
    refrain from discussing the evolution of languages. One pragmatic
    reason is that we do not want to give the impression that we know
    how Oracle should handle the JLS. Obviously, Oracle (and other owners of
    language documentation) have a quality problem, but we know, based
    on our work, for example, in the Cobol ISO WG, that language
    documentation is an extremely complex process. So everything we
    could possible say, we feel, would be naive, incomplete, and
    perhaps even offending. But again, we pursue this direction of
    research at other levels. The abovementioned paragraph at the end
    of Section 4 also refers to a paper on the subject. To summarize,
    we deliberately decided to not mix the general yet certainly
    debatable guidelines for language evolution and language
    documentation evolution with the concrete data we had to report on
    this study.%
  }

\qa{``Abbreviated as formatting issue''%
}{%
  Done.%
}

\end{itemize}

\medskip

\item Review 4

\begin{itemize}

  \qa{I have a few comments that can be used to improve the paper: In
    Section 3, you mention a set of operators. It's not clear whether
    these operators are specific for JLS or are they generalizable to
    other cases. If they are specific, how should I define a set of
    operators for a specific language (e.g., suppose I have to do the
    same for several COBOL or C dialects). Probably it would be useful
    to summarize in a table a sort of operator taxonomy.%
  }{%
    The operators are independent of the language modeled by the
    grammars subject to transformation. The metasyntax and semantics
    of transformations only depends on the metasyntax of grammars.
    The choice of operators implies a certain bias towards an
    application scenario. For instance, if we only had refactoring
    operators, convergence was not fully covered. We have added
    systematic explanations for all relevant transformation operators
    to the paper. We have also compared the present paper's suite with
    prior art.}

  \qa{Page 4: can you please better explain what the term "massage"
    means in the grammar terminology? At the end it is clear however I
    guess the reader is not used to such a term, while for instance
    other terms as "factoring" are more common.}{%
    Examples and formalization have been added; see App. B, for example.
  }

  \qa{I think the tricky part is how to decide what operator apply
    before and what after. Can you provide some guideline on how to
    proceed? It looks like this is a problem where the engineer has to
    search among possible solutions and sometimes stepping back
    because the application of an operator before the other is
    changing the grammar in the wrong direction.%
  }{%
    Yes, very well spotted. We have tried to improve the paper to
    address this question; see Section 2 on the method; see Section
    2.4 and Section 2.5 in particular. We provide some advice. The
    main idea is that the order does not matter for most of the
    process. That is, as long as you do refactoring, the only
    requirement is that you should reduce the number of
    differences. Once you start doing the few transformations for
    fixing inconsistencies, we do not provide real guidance. One could
    accidentally damage the grammar. In practice, there is no real
    problem, in our experience, but the door is open for making
    mistakes. So this is one of key subjects for future work.}

  \qa{What does it happen when the grammar adds a new terminal? A
    classical example is the "enum" keyword between Java grammars 1.4
    and 1.5, I remember I had to deal with that to make a grammar able
    to parse both versions of the language%
  }{%
    We have picked up this specific example (``enums'') in the new
    Sec. 2. Essentially, the idea is to \emph{add} an alternative to
    an existing nonterminal's definition.%
  }

  \qa{Section 4.1: you mention a tool-supported grammar
    comparison. How is it made? What kind of tool did you use?%
  }{%
    We are using a technology that is part of the package for grammar
    convergence. This aspect is now fully described and demonstrated
    in the paper; see Section 2.%
  }

  \qa{Related work: you might want to mention other papers describing
    approaches aimed at recovering grammars, e.g.: Oscar Nierstrasz,
    Markus Kobel, Tudor Gîrba, Michele Lanza, Horst Bunke:
    Example-Driven Reconstruction of Software Models. CSMR 2007:
    275-286; Massimiliano Di Penta, Pierpaolo Lombardi, Kunal Taneja,
    Luigi Troiano: Search-based inference of dialect grammars. Soft
    Comput. 12(1): 51-66 (2008)%
  }{%
    Thanks for the references. They are indeed all relevant. We have
    included them, and we have generally extended the related work
    discussion to include all work on grammar recovery, in particular,
    and on grammar engineering, in general.%
  }

  \qa{Conclusions: you mention the productivity of engineers. This is
    a very important point. To what extend did the process you
    described help to improve productivity? How long did it take to
    perform the tasks described in the case study?%
  }{%
    There is no base for comparison. When we talk about improved
    productivity, then we envisage to improve the productivity of
    grammar convergence relative to what it is now (without inference
    of transformations, without an IDE, etc.). However, grammar
    convergence is not done by anyone or with anyone else's method.
    Hence, we do not see base for comparison. We could pick a
    hypothetical base: such as code inspection for grammars. That is,
    we could wonder whether code inspection would be more productive
    in recovering grammar relationships or in finding inconsistencies.
    However, this does not make much sense because a) obviously
    substantial efforts at Sun et al.\ have not been sufficient to
    avoid these inconsistencies that we have found. Without a method
    like grammar convergence, there is not even any way how someone
    could represent grammar relationships. We ask you to have a look
    at the revised paper, and let us know of any ideas for a possible
    comparison of productivity. We simply hope that the question does
    not come up any more with this revision.%
  }

\end{itemize}

\end{itemize}

\noindent
\textbf{With best regards,}

\noindent
\textbf{Ralf L\"ammel \& Vadim Zaytsev}

\newpage


==> examples/xbgf.tex <==
\begin{minipage}{\textwidth}
\begin{tabular}{ll}
{\begin{lstlisting}[language=pp]
sequence:
		(transformation | atomic)*
atomic:
		transformation+
transformation:
		folding-unfolding-transformation
		refactoring-transformation
		increasing-transformation
		decreasing-transformation
		concrete-revising-transformation
		abstract-revising-transformation
		renaming-transformation
		decorative-transformation
		reroot::(root::nonterminal*)
		dump::EPSILON
folding-unfolding-transformation:
		unfold::(nonterminal in::scope?)
		fold::(nonterminal in::scope?)
		inline::nonterminal
		extract::(production in::scope?)
		abridge::production
		detour::production
		unchain::production
		chain::production
refactoring-transformation:
		massage::(expression expression in::scope?)
		distribute::scope
		factor::(expression expression in::scope?)
		deyaccify::nonterminal
		yaccify::(production+)
		eliminate::nonterminal
		introduce::(production+)
		import::(production+)
		vertical::scope
		horizontal::nonterminal
		equate::(align::nonterminal with::nonterminal)
		rassoc::production
		lassoc::production
\end{lstlisting}}
&
{\begin{lstlisting}[language=pp]
increasing-transformation:
		addV::production
		addH::marked-production
		appear::marked-production
		widen::(expression expression in::scope?)
		upgrade::(marked-production production)
		unite::(add::nonterminal to::nonterminal)
decreasing-transformation:
		removeV::production
		removeH::marked-production
		disappear::marked-production
		narrow::(expression expression in::scope?)
		downgrade::(marked-production production)
concrete-revising-transformation:
		abstractize::marked-production
		concretize::marked-production
		permute::production
abstract-revising-transformation:
		define::(production+)
		undefine::(nonterminal+)
		redefine::(production+)
		inject::marked-production
		project::marked-production
		replace::(expression expression in::scope?)
renaming-transformation:
		renameL::(from::label to::label)
		renameN::(from::nonterminal to::nonterminal)
		renameS::(in::label? from::selector to::selector)
		renameT::(from::terminal to::terminal)
decorative-transformation:
		designate::production
		unlabel::label
		deanonymize::marked-production
		anonymize::marked-production
marked-production:
		production
scope:
		label | nonterminal
\end{lstlisting}}
\end{tabular}
\end{minipage}


==> leftover.tex <==
In practice, it is common that each source requires some (possibly
trivial) transformation steps to finalize the extraction process
properly, to account for previously known inconsistencies and to fix
other issues that are apparent without comparison (based on, say,
grammar static analysis). In the present JLS case study, we 


derived
targets always from two grammars, and we always ???

 grammar of the two~---~in such case the
common denominator is derived from it by those preparatory
transformation steps. When another issue arises in the favored grammar
as a result of transforming the non-favored one, we need to update the
preparatory transformation scripts and refactor the accumulated
transformations to deal with the changed common denominator.

